The Two-Component Becker-D\"oring System: Basic Properties

The two-component Becker-D\"oring model is a two-dimensional coagulation-fragmentation equation that describes the dynamics of clusters built from two different types of monomers growing and shrinking through monomer interaction. We show the existence and mass conservation of solutions and give a partial result regarding uniqueness. Furthermore, we prove under the assumption of detailed balance the entropy equation, followed by a detailed study of the equilibrium states and relative entropies. We can determine the minimum of all relative entropies under sequences of fixed Type I and Type II masses and fully describe the minimising sequences in the weak* topology.

==> proofs/steadyStateDB.tex <==
If $\rho = 0$ or $\sigma = 0$, any solution has to satisfy $z=0$ and $w=0$ respectively.
But $\rho(\cbar^{z,0})$ and $\sigma(\cbar^{0,w})$ are monotone in $z$ and $w$ respectively, so there is at most one solution.

Now consider $\rho_0,\sigma_0>0$. And let $(z,w) \in \Ex$ and $(u,v) \in \Ex$ with $\rho(\cinfzw) = \rho_0 = \rho(\cinfuv)$ and  $\sigma(\cinfzw) = \sigma_0 = \sigma(\cinfuv)$. Then, we clearly have $z,w,u,v > 0.$ With this we can calculate
\begin{equation*}
  \begin{split}
    0 \le H[u,v|z,w] &= \ln\left( \frac u v \right)\rho(\cinfuv) + \ln\left( \frac v w\right) \sigma(\cinfuv) + \sumrs \cinfzw\rs -\cinfuv\rs\\
    &= \ln\left( \frac u v \right)\rho(\cinfzw) + \ln\left( \frac v w\right) \sigma(\cinfzw) + \sumrs \cinfzw\rs -\cinfuv\rs = -H[z,w|u,v] \le 0.
  \end{split}
\end{equation*}
So $H[u,v|z,w] = 0$, but since $\Psi(x) \ge 0$, we already get 
\[ \cinfzw\rs \Psi\left(\frac {\cinfuv\rs}{\cinfzw\rs}\right) = 0 \text{ for all } r,s.\]Finally, $\Psi(x) > 0$ for all $x\neq1$ implies $\cinfzw\rs = \cinfuv\rs$ for all $r+s \ge 0.$

